DAGE: DAG Query Answering via Relational Combinator with Logical Constraints

Predicting answers to queries over knowledge graphs is called a complex reasoning task because answering a query requires subdividing it into subqueries. Existing query embedding methods use this decomposition to compute the embedding of a query as the combination of the embedding of the subqueries. This requirement limits the answerable queries to queries having a single free variable and being decomposable, which are called tree-form queries and correspond to the $\mathcal{SROI}^-$ description logic. In this paper, we define a more general set of queries, called DAG queries and formulated in the $\mathcal{ALCOIR}$ description logic, propose a query embedding method for them, called DAGE, and a new benchmark to evaluate query embeddings on them. Given the computational graph of a DAG query, DAGE combines the possibly multiple paths between two nodes into a single path with a trainable operator that represents the intersection of relations and learns DAG-DL from tautologies. We show that it is possible to implement DAGE on top of existing query embedding methods, and we empirically measure the improvement of our method over the results of vanilla methods evaluated in tree-form queries that approximate the DAG queries of our proposed benchmark.

==> Problem_Definition.tex <==
\label{Problem Definition}
We present the definition of the DAG query answer prediction task. We begin by formally defining the DAG query using logic theory.
\begin{mydef}[two-variable query]
    The set of the two-variable queries is the smallest $\Phi$ that satisfies the following:
    \begin{itemize}
        \item for $\phi(x,y) = r(x,y)$, where x and y are free variables, itself and its negation $r(x,y)$, $\neg r(x,y)$ $\in \Phi$,
        \item given an atomic query $\phi(x)$ and a two-variable query $\psi(x,y)$, then $\phi(x) \land \psi(x,y) \in \Phi$,
        \item given a one-variable query $\phi(\cdot)$ and a two variable $\psi(x,y)$, then $\phi(x) \land \psi(x,y) \in \Phi$ and $\phi(y) \land \psi(x,y) \in \Phi$,
        \item given two-variable queries $\phi(y,x)$ and $\psi(y,x)$, then $\phi(y,x) \land \psi(y,x) \in \Phi$ and $\exists z. (\phi(y,z ) \land \psi(z,x) \in \Phi$.
    \end{itemize}
\end{mydef}

\begin{mydef}[$\text{DAG}$ Query]
\label{DAG query}
The set of the $DAG$ queries is the smallest set $\Phi_{DAG}$ that satisfies the following:
    \begin{itemize}
        \item for atomic query $phi(x)$, itself and its negation $\neg \phi(x) \in \Phi_{DAG}$,
        \item if $\phi \in \Phi_{DAG}$, $x$ is a bounded variable and $y$ is a free variable, then $\exists x. \phi(y) \in \Phi_{DAG}$,
        \item given a two variable query $\psi(x,y)$ and $\phi \in \Phi_{DAG}$, then $\exists y. (\phi(y) \land \psi(y, x) ) \in \Phi_{DAG}$,
        \item if $\phi, \psi \in \Phi_{DAG}$, then $\phi(x) \land \psi(x), \phi(x) \lor \psi(x) \in \Phi_{DAG}$.
    \end{itemize}
\end{mydef}
Then, we outline the query answer prediction task over DAG queries.
\begin{mydef}[$\text{DAG}$ Query Answer Prediction Task]
Given a knowledge graph G and {}
\end{mydef}




